CircuitLens: Reasoning Circuits as Data Selection Signals for Reinforcement Learning with Verifiable Rewards

Reinforcement learning with verifiable rewards (RLVR) is sensitive to which problems a model trains on, yet existing selection criteria--difficulty filtering, hand-curation, reward-trajectory scoring--assess data value as an intrinsic property of problems, independent of the model that will learn from them. We introduce Circuit Reasoning Score (CRS), a selection signal derived from 46 reasoning-sensitive attention heads identified via contrastive ablation, computed in a single forward pass on the frozen base model without reward labels or rollouts. CRS runs against the intuitive hypothesis that stronger reasoning-circuit engagement produces better training data: on Qwen2.5-Math-7B, the lowest-engagement decile improves over random selection on three medium-difficulty benchmarks (GSM8K +2.0 pp, OlympiadBench +1.6 pp, Minerva +2.9 pp), while the highest-engagement decile gains less and is indistinguishable from the middle decile. The advantage has boundary conditions: on a domain-curated pool no selection method separates from the others; at 1.5B scale the useful direction differs; and the lowest-reward training condition produces the strongest downstream generalization. Within the Qwen2.5-Math settings tested, RLVR data selection appears regime-dependent rather than reducible to a static ranking of problem quality.

==> tables/tab_datasets.tex <==
\begin{table}[t]
\centering
\caption{Datasets used in each experimental stage.}
\label{tab:datasets}
\begin{tabular}{llrl}
\toprule
\textbf{Stage} & \textbf{Dataset} & \textbf{N} & \textbf{Purpose} \\
\midrule
Circuit ID (Stage 3) & MATH-500 & 400/boot & Reasoning probes \\
                     & GS··M8K (shortest) & 100 & Trivial controls \\
\midrule
CRS Scoring (Stage 5) & DAPO-Math-17K & 17{,}186 & Candidate pool \\
\midrule
RLVR Training (Stage 7) & CRS top-10\% & 1{,}718 & Selected subset \\
                        & Random 10\% & 1{,}718 & Baseline \\
\midrule
Evaluation (Stage 9) & MATH-500 & 500 & Primary benchmark \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_hyperparams.tex <==
\begin{table}[t]
\centering
\caption{GRPO training hyperparameters.}
\label{tab:hyperparams}
\begin{tabular}{ll}
\toprule
\textbf{Parameter} & \textbf{Value} \\
\midrule
Base model & Qwen2.5-Math-7B \\
Algorithm & GRPO \\
Learning rate & $5 \times 10^{-7}$ \\
Warmup steps & 10 \\
Temperature & 0.7 \\
Num. generations per prompt & 16 \\
Max completion length & 4096 tokens \\
Per-device batch size & 4 \\
Gradient accumulation & 4 \\
Effective batch (prompts/step) & 16 \\
GPUs & 8 $\times$ A100-80GB \\
Precision & bf16 \\
Reward & Binary correctness \\
Framework & TRL 1.3.0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_main_results.tex <==
\begin{table}[t]
\centering
\caption{Main results: MATH-500 pass@1 after GRPO training on different data subsets. All conditions use the same total training tokens (token-matched).}
\label{tab:main_results}
\begin{tabular}{lcrr}
\toprule
\textbf{Selection Method} & \textbf{Data \%} & \textbf{MATH-500 pass@1} & \textbf{$\Delta$ vs Random} \\
\midrule
ReasonSelect (CRS top-10\%) & 10\% & \textit{pending} & --- \\
Random 10\% & 10\% & \textit{pending} & 0.0 \\
Bottom CRS 10\% (neg. ctrl) & 10\% & \textit{not yet run} & --- \\
Full data & 100\% & \textit{not yet run} & --- \\
\midrule
\multicolumn{4}{l}{\footnotesize Base model (no RLVR): $\sim$30\% estimated from pass@1 sanity check.} \\
\bottomrule
\end{tabular}
\end{table}

